RuleExplorer: A Scalable Matrix Visualization for Understanding Tree Ensemble Classifiers

The high performance of tree ensemble classifiers benefits from a large set of rules, which, in turn, makes the models hard to understand. To improve interpretability, existing methods extract a subset of rules for approximation using model reduction techniques. However, by focusing on the reduced rule set, these methods often lose fidelity and ignore anomalous rules that, despite their infrequency, play crucial roles in real-world applications. This paper introduces a scalable visual analysis method to explain tree ensemble classifiers that contain tens of thousands of rules. The key idea is to address the issue of losing fidelity by adaptively organizing the rules as a hierarchy rather than reducing them. To ensure the inclusion of anomalous rules, we develop an anomaly-biased model reduction method to prioritize these rules at each hierarchical level. Synergized with this hierarchical organization of rules, we develop a matrix-based hierarchical visualization to support exploration at different levels of detail. Our quantitative experiments and case studies demonstrate how our method fosters a deeper understanding of both common and anomalous rules, thereby enhancing interpretability without sacrificing comprehensiveness.

==> 6-evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}


\begin{table*}[t]
\setlength{\tabcolsep}{8.5pt}
\vspace{-0.5mm}
\caption{Performance comparison between our method and the baseline methods in terms of fidelity and average anomaly score.} 
\resizebox{\linewidth}{!}{
\begin{tabular}{cccccccccccccc} 
\toprule 
\multirow{2}{*}{Dataset} & \multirow{2}{*}{\#Classes} & \multirow{2}{*}{\lizhenrev{\#Attributes}} & \multirow{2}{*}{\#Samples} & \multirow{2}{*}{Model} & \multirow{2}{*}{\lizhenrev{\#Rules}} & \multicolumn{2}{c}{Ours} & \multicolumn{2}{c}{RuleMatrix} & \multicolumn{2}{c}{HSR} & \multicolumn{2}{c}{Node harvest} \\ 
\cmidrule(lr){7-8} \cmidrule(lr){9-10} \cmidrule(lr){11-12} \cmidrule(lr){13-14}
~ & ~ & ~ & ~ & ~ & ~ & Fidelity & AS & Fidelity & AS & Fidelity & AS & Fidelity & AS \\
\midrule
\multirow{2}*{Credit Card} & \multirow{2}*{2} & \multirow{2}*{\lizhenrev{14}} & \multirow{2}*{690} & RF & \lizhenrev{7,085} & \textbf{0.9538} & \textbf{0.1309} & 0.9503 & 0.0880 & 0.9264 & 0.0000 & 0.9300 & 0.0473\\
~ & ~ & ~ & ~ & GBT & \lizhenrev{2,126} & \textbf{0.9249} & \textbf{0.1271} & 0.9075 & 0.0735 & 0.8682 & 0.0846 & 0.9017 & 0.0042\\
\hline
\multirow{2}*{Wine Quality} & \multirow{2}*{2} & \multirow{2}*{\lizhenrev{11}} & \multirow{2}*{1,599} & RF & \lizhenrev{28,116} & \textbf{0.8725} & 0.1432 & 0.8665 & 0.0689 & 0.7484 & 0.0000 & 0.5175 & \textbf{0.1660}\\
~ & ~ & ~ & ~ & GBT & \lizhenrev{7,474} & \textbf{0.8350} & \textbf{0.0974} & 0.8065 & 0.0329 & 0.7368 & 0.0000 & 0.8275 & 0.0299\\
\hline
\multirow{2}*{Crime} & \multirow{2}*{2} & \multirow{2}*{\lizhenrev{127}} & \multirow{2}*{1,994} & RF & \lizhenrev{12,576} & \textbf{0.9178} & \textbf{0.1999} & 0.9042 & 0.0203 & 0.8910 & 0.0000 & 0.8577 & 0.1602\\
~ & ~ & ~ & ~ & GBT & \lizhenrev{4,322} & \textbf{0.9118} & \textbf{0.1152} & 0.8986 & 0.0119 & 0.8368 & 0.0000 & 0.8978 & 0.0489\\
\hline
\multirow{2}*{Abalone} & \multirow{2}*{4} & \multirow{2}*{\lizhenrev{8}} & \multirow{2}*{4,177} & RF & \lizhenrev{23,500} & \textbf{0.8392} & \textbf{0.1247} & 0.8243 & 0.0085 & 0.6695 & 0.0081 & N/A & N/A\\
~ & ~ & ~ & ~ & GBT & \lizhenrev{11,810} & \textbf{0.8967} & 0.1263 & 0.8268 & 0.1231 & 0.5715 & \textbf{0.3553} & N/A & N/A\\
\hline
\multirow{2}*{Obesity} & \multirow{2}*{7} & \multirow{2}*{\lizhenrev{16}} & \multirow{2}*{2,111} & RF & \lizhenrev{19,490} & \textbf{0.8561} & \textbf{0.1732} & 0.7720 & 0.0138 & 0.7277 & 0.0683 & N/A & N/A\\
~ & ~ & ~ & ~ & GBT & \lizhenrev{30,458} & \textbf{0.9470} & \textbf{0.2309} & 0.8394 & 0.0004 & 0.7233 & 0.0084 & N/A & N/A\\
\hline
\multirow{2}*{Dry Bean} & \multirow{2}*{7} & \multirow{2}*{\lizhenrev{16}} & \multirow{2}*{13,611} & RF & \lizhenrev{6,209} & \textbf{0.9738} & \textbf{0.2829} & 0.9702 & 0.0032 & 0.8726 & 0.0193 & N/A & N/A\\
~ & ~ & ~ & ~ & GBT & \lizhenrev{52,455} & \textbf{0.9151} & \textbf{0.3032} & 0.9151 & 0.0946 & 0.8369 & 0.2360 & N/A & N/A\\
\bottomrule
\end{tabular}
}
\begin{tablenotes}
\item {RF}: random forest. {GBT}: gradient boosted tree.
{AS}: average anomaly score. Node harvest cannot handle multi-classification datasets.
\end{tablenotes}
\label{tab:result}
\end{table*}

We \jwrevision{first} conducted a quantitative experiment to evaluate the effectiveness of the anomaly-biased model reduction method. %and 
\jwrevision{We} then presented two case studies to showcase how {\system} helps domain experts understand the decision logic of tree ensemble classifiers and improve them.
\looseness=-1

\subsection{Quantitative Experiment}


\noindent\textbf{Datasets}.
We conducted the quantitative experiment on six datasets from the UCI Machine Learning Repository~\cite{asuncion2007uci}, as used in previous works~\cite{ming2018rulematrix, yuan2024visual}, including three binary classification datasets (Credit Card, Wine Quality, Crime) and three multiple classification ones (Abalone, Obesity, Dry Bean). \lizhenrev{The number of attributes across these datasets ranged from 8 to 127, while the number of samples ranged from 690 to 13,611.
The diverse characteristics of these datasets enable a robust evaluation across various tasks and dataset scales.}\looseness=-1
% The sizes of these datasets range from hundreds to several thousands.

\noindent\textbf{Baseline methods}.
We selected three baseline methods, including
two model surrogate methods, RuleMatrix~\cite{ming2018rulematrix} and HSR~\cite{yuan2024visual}, and a state-of-the-art model reduction method, node harvest~\cite{meinshausen2010node}.
RuleMatrix generates a sequential rule list, while HSR generates a hierarchical rule set.
Different from these two methods, node harvest directly extracts the rules from the original model rather than generating new ones.
However, it cannot be used in multi-class classification.

\noindent\textbf{Measures}.
We evaluated the quality of the methods from two aspects.
% First, \emph{fidelity} measures the ability of the generated rule sets to preserve the behavior and predictive accuracy of the original model.
First, \emph{fidelity} measures the ability to preserve the behavior and predictive accuracy of the original model.
It is defined as the ratio of the samples with the same predictions produced by the generated rule sets and the original model. 
% Second, the \emph{average anomaly score} of the generated rule sets evaluates the ability of the model reduction method to preserve anomalous rules.
Second, the \emph{average anomaly score} evaluates the ability to preserve anomalous rules.


\noindent\textbf{Experiment settings}.
To demonstrate the generalizability of our method to different tree ensemble classifiers, we conducted experiments
on random forest models and gradient boosted tree models.
Each dataset was partitioned into a 75\% training set and a 25\% test set.
We first trained each model on the training set, 
\lizhen{ resulting in models with rule counts ranging from 2,126 (LightGBM on credit card dataset) to 52,455 (LightGBM on drybean dataset). }
\lizhenrev{This wide range of rule numbers ensures a thorough evaluation across different levels of model complexity}.
%\lizhen{resulting in models containing thousands to tens of thousands of rules}.
Then, we performed model reduction to approximate the predictions on the training set.
\lizhen{ All methods are required to select 80 rules (consistent with Sec. IV) for this approximation. }
The fidelity was calculated on the test set, and the average anomaly score was calculated on the generated rule set.
% \weikai{The parameters $\xi$ and $\lambda$ are simultaneously determined using grid search to strike a balance between fidelity and anomaly detection.}
We ran five trials for each setting to reduce the effect of randomness.

% After discussing with the experts, we set $M$ (the number of the generated rules) to 80 in our method.
% $\xi$ is determined by a grid search to achieve the highest fidelity with $\lambda$ as 0.
% $\lambda$ is also determined by a grid search for the highest average anomaly score with a tolerance of $1\%$ drop of the highest fidelity.
% For the method used in RuleMatrix and node harvest, we also set the number of the generated rules to 80 (the same as $M$ in our method).
% For HSR, since it could not limit the number of the generated rules, 
% we determined its parameters by a grid search for the highest fidelity.

\noindent\textbf{Results}.
Our results are summarized in Table~\ref{tab:result}.
Our method achieved the highest fidelity across all cases,
and also achieved higher average anomaly scores than the baseline methods except in two cases. 
On the Wine Quality dataset, node harvest obtained a higher average anomaly score for the random forest model,
while on the Abalone dataset, HSR obtained a higher average anomaly score for the gradient boosted model.
However, the fidelity scores achieved in these two cases are significantly lower ($0.5175$ and $0.5715$), indicating the corresponding rule sets failed to approximate the behavior of the original model.
In contrast, our method achieved the highest fidelity and the second-highest average anomaly scores. 
This demonstrates that our method can strike a balance between fidelity and the preservation of anomalous rules.


\subsection{Case Studies}
We conducted two case studies to show the usefulness of {\system} in explaining and diagnosing tree ensemble classifiers.\looseness=-1

\subsubsection{Credit Card Approval}

In this case study, we collaborated with E$_1$ and E$_2$ to illustrate how {\system} improves the understanding and diagnosis of the model to approve credit card applications.
E$_1$ is a bank account manager with two years of work experience, who aims to increase credit card approval rates while minimizing the risk of defaults.
E$_2$ is a data scientist responsible for developing the credit card approval model and improving its performance.
\weikai{\jwrevision{Both E$_1$ and E$_2$}
have participated in the interview for collecting design goals in Sec.~\ref{sec:overview}}.
\lizhenrev{During the study, E$_1$ interacted with the system to explore and identify potential model issues, while E$_2$ helped explain the underlying causes of these findings from a machine learning perspective and suggested ways to improve the model.}
The study used the Australian Credit Approval dataset~\cite{australian_credit_approval}, which consists of 690 samples, each representing a credit card applicant with 16 attributes and a label indicating approval or rejection.
The dataset includes 307 ``\textbf{approved}'' samples and 383 ``\textbf{rejected}'' samples.
These samples were randomly divided into training and test data with a ratio of 75\% and 25\%, respectively.
To comprehensively evaluate the model, E$_2$ used Synthetic Data Vault~\cite{SDV} to augment the test data based on its distribution and labeled the new test samples in collaboration with E$_1$.
\lizhenrev{The detailed augmentation process can be found in the supplemental material.}
After the augmentation, there are 500 samples in the test data.
A random forest model \lizhen{with 200 trees and a maximum depth of 10} has been trained on this dataset with the scikit-learn library~\cite{scikit-learn}.
The trained model includes \textbf{7,085} rules and achieves an accuracy of 83.60\%.


\noindent\textbf{Overview}.
Initially, E$_1$ investigated the attributes frequently used in the extracted rules to see whether the decision-making process was reasonable.
As shown in Fig.~\ref{fig:teaser}A, the attributes that describe income and credit status, such as \emph{PriorDefault}, \emph{Job}, \emph{Income}, \emph{Years Employed}, are frequently used and thus appear in the first few columns.
This observation aligns with his experience, as these attributes are more important in credit card approval than those less frequently used 
attributes like \emph{Gender} and \emph{DriverLicenses}.
Subsequently, E$_1$ examined the rules to see how these frequently used attributes influenced model predictions.
He focused on two types of rules: common \jwrevision{rules} and anomalous rules.
% Common rules have high coverage and low anomaly scores, which reveal the general prediction behavior of the model.
% In contrast, anomalous rules have low coverage but high anomaly scores, which often disclose potential flaws and exceptional scenarios in the model.

\begin{figure}[t]
\centering
\includegraphics[width=1\linewidth]{figures/priordefault_revision.pdf}
\caption{Anayzing the rules that utilize the attribute \emph{PriorDefault}:
% \lizhen{ rules with no prior defaults determine rejection (A) or approval (B) based on additional conditions, while those with prior defaults consistently predict rejection (C). Zoom in to further analysis (D). }
\lizhen{rules with no prior defaults may reject (A) or approve (B) credit card applications, while those with prior defaults consistently reject applications (C). Zoom in region C to examine the neighborhood (D). }
} 
\label{fig:case1-prior-default}
\end{figure}




\noindent\textbf{Analyzing common rules}.
By default, the rules are sorted in descending order of their coverage.
E$_1$ first analyzed common rules \jwrevision{(rules with higher coverage)} and found that most of them used the attribute \emph{PriorDefault} (Fig.~\ref{fig:teaser}B).
He wanted to examine how \emph{PriorDefault} influenced the model predictions.
To this end, he clicked on the header of \emph{PriorDefault}, and the rules were grouped based on their conditions on this attribute.
\jwrevision{There are three groups.} 
%The rules were divided into three parts 
(Fig.~\ref{fig:case1-prior-default}).
At the top, the rules with the condition of no prior defaults made predictions of ``rejected'' (Fig.~\ref{fig:case1-prior-default}A).
\lizhen{
\weikai{The matrix reordering algorithm reveals several patterns,}
such as low income, few years employed, or low credit scores, which accounted for the rejection.}
% The pattern formed by similar conditions reflects that these rules typically include other negative conditions, 
%These rules often included other negative conditions, such as low income, low credit scores, or unemployment, which accounted for the rejection.
%On the contrary, in 
\jwrevision{In} the middle, the rules with the condition of no prior defaults made predictions of 
``approved'' (Fig.~\ref{fig:case1-prior-default}B).
\jwrevision{Compared to the group at the top,} 
these rules had additional positive conditions, 
\lizhen{such as a certain income level or being older, indicating a lower risk of default and a more stable status.}
E$_1$ regarded the behavior (Fig.~\ref{fig:case1-prior-default}A and B) as reasonable, since the condition of no prior defaults cannot directly lead to the approval, and it should be combined with additional conditions for further consideration.
At the bottom, the rules with the condition of prior defaults consistently led to predictions of ``rejected'' (Fig.~\ref{fig:case1-prior-default}C).
%After zooming into this region and examining its neighborhood
\lizhen{E$_1$ selected these rules and zoomed into their neighborhood in the dynamic hierarchy. 
As a result, he found that all these rules resulted in ``rejected'' (Fig.~\ref{fig:case1-prior-default}D).
}
% \lizhen{providing a more focused view of the model's behavior.}
Since there are some real-world cases where applicants with prior default records are still approved, E$_1$ was curious why this was not reflected in these rules, and consulted with E$_2$. E$_2$ explained that a credit card approval model typically rejects all applicants with prior default records in realistic scenarios and leaves disputed cases for manual processing.
\lizhen{E$_1$ agreed with this strategy, as applicants with default records pose a higher credit risk.} 
To summarize, E$_1$ was satisfied with the behavior of the rules utilizing \emph{PriorDefault}.
Similarly, E$_1$ analyzed other frequently used attributes, including \emph{Job}, \emph{Income}, \emph{Years Employed}, and acknowledged that these attributes were properly employed to make predictions. 


E$_1$ continued to examine common rules and noticed a rule that had significantly lower confidence than the rules with similar coverage (Fig.~\ref{fig:teaser}C).
The low confidence indicated that this rule covered many mispredicted samples.
Therefore, he examined its covered samples. %to find the reason. Upon examination, he 
\jwrevision{He} found that these samples shared some negative conditions (Fig.~\ref{fig:teaser}D), including unemployment, missing credit scores, lack of income, and having prior default records.
Although these samples were labeled as ``approved'' (Fig.~\ref{fig:teaser}E), E$_1$ suspected \jwrevision{they} %that they 
should be rejected given those negative conditions.
He then filtered the samples with such negative conditions and found that they were mostly labeled as ``rejected.''
This indicated that there were inconsistent approval criteria in the training data.
He raised this issue with E$_2$, and E$_2$ commented that such inconsistency harmed the model training and led to performance degradation.
Therefore, E$_1$ unified the approval criteria in these samples and corrected their labels to be ``rejected.''
By retraining the model on the corrected data, the accuracy increased from 83.60\% to 86.20\%, and the prediction confidence increased from 0.7403 to 0.7423.



\begin{figure}[t]
\centering
\includegraphics[width=1\linewidth]{figures/all_anomaly.pdf}
\caption{Analyzing the top-2 rules with the highest anomaly scores: 1)
\lizhen{the analysis of the first rule (A$_1$), its neighbors (B$_1$), and the associated sample (C$_1$) reveals a labeling error; 2) the analysis of the second rule (A$_2$), its sample distribution (B$_2$), and information from the \textit{attribute \jwrevision{and info} views} (C$_2$, D$_2$) confirms a spurious association.}}
\vspace{-4mm}
\label{fig:case1-anomaly}
\end{figure}

\noindent\textbf{Analyzing anomalous rules}.
To identify potential flaws in the model,
E$_1$ turned to analyze the anomalous rules.
He sorted the rules according to their anomaly scores.
The low coverage of the anomalous rules suggested that they were learned from only a few samples.
E$_1$ started his analysis by examining the rule with the highest anomaly score.
As shown in Fig.~\ref{fig:case1-anomaly}A$_1$, this rule suggests approval for young, single, unemployed applicants with a medium-to-low income.
These conditions were mostly neutral or negative, which should not lead to an approval.
He zoomed in to examine its neighborhood
and observed that they shared few conditions (Fig.~\ref{fig:case1-anomaly}B$_1$), which also indicated that its behavior differed a lot from other rules.
To analyze why this rule was learned, he clicked on it and examined its covered samples. As shown in Fig.~\ref{fig:case1-anomaly}C$_1$, it covered only an 18-year-old applicant with a 10-year work experience (\#321).
%Due to the spurious information 
\jwrevision{It is suspicious} that an 18-year-old %person had 
\jwrevision{has} a 10-year work experience. E$_1$ confirmed that this applicant should not be approved \jwrevision{and corrected its label to ``rejected''.} 
%Such a label error in the training sample led to this rule. Therefore, he decided to correct its label to ``rejected.''

Subsequently, E$_1$ examined the rule with the second-highest anomaly score.
This rule suggested approval for applicants with some debt, having a low credit score, having a driver's license, and having a specific job of type \#7 (Fig.~\ref{fig:case1-anomaly}A$_2$). 
As these conditions were primarily neutral or negative, E$_1$ \jwrevision{doubted the approval decision for these applicants.} %suspected 
%whether these applicants should be approved.
Therefore, he checked the samples covered by this rule and realized that most of the applicants had no prior default records and a certain level of income (Fig.~\ref{fig:case1-anomaly}B$_2$).
E$_1$ believed %that 
these positive conditions were the real reason for the approval.
By filtering %the 
samples with such positive conditions using the scented widgets in the \textit{attribute view} (Fig.~\ref{fig:case1-anomaly}C$_2$), he found that most of them (\lizhenrev{98.26\%}) are approved (Fig.~\ref{fig:case1-anomaly}D$_2$).
Thus, he \jwrevision{suspected} %concluded 
that this rule occurred because of the spurious association between the irrelevant conditions and the approval decision in these covered samples (Fig.~\ref{fig:case1-anomaly}A$_2$).
\weikai{E$_1$ then discussed this issue with E$_2$.
E$_2$ \jwrevision{considered}
%pointed out that 
adding more diverse samples, especially %applicants 
\jwrevision{those} that meet the conditions of this rule but get rejected, %will 
\jwrevision{would} mitigate this spurious association.
%Therefore, E$_2$ 
\jwrevision{He thus} generated \jwrevision{more} %additional 
samples using data augmentation, and E$_1$ validated these samples to ensure they accurately reflected real-world scenarios.}
% After studying this spurious association, \lizhen{which is often caused by data bias}, E$_2$ proposed to address through data augmentation, \lizhen{explaining that adding more diverse samples can help mitigate the data bias that leads to the spurious association}.
% Specifically, he generated additional samples of rejected applicants who met the conditions of this rule but lacked a certain level of income or had prior default records.
% \lizhen{E$_1$ then validated these samples to ensure they accurately reflected real-world scenarios.}


They analyzed other anomalous rules with the top-20 anomaly scores and found 1 more rule caused by label error and 15 more rules caused by spurious associations.
Similarly, they corrected the label error and augmented the training samples.
After retraining the model, the accuracy increased from 86.20\% to 88.60\%, and the average prediction confidence increased from 0.7423 to 0.7630.
The average anomaly score of the rules also decreased from 0.0547 to 0.0493.


\begin{figure*}[t]
  \centering
    \includegraphics[width=1\linewidth]{figures/stock_revision.pdf}
     \vspace{-2mm}
        \caption{
        %Analyzing rules for quantitative stock trading: (a) the initial model; (b) the model after removing the attributes causing biased predictions.
        \lizhen{%\jwrevision{Analyzing rules for quantitative stock trading: (a) in the initial model; (b) after removing attributes that cause biased predictions; (c) after adding more useful attributes for predicting ``Increase''; and (d) in the neighborhood of selected rules.}
        Analyzing rules for quantitative stock trading: (a) in the initial model, rules with lower \textit{KLEN} typically indicate ``Stable'' (A), except for one outlier (B); (b) after removing attributes that cause biased predictions, \textit{STD60} was found to be crucial for predicting an ``Increase'' (C, D); (c) after adding more useful attributes for predicting ``Increase'', the importance of \textit{STD60} decreased (E), while \textit{NATR} became the most important attribute (F), which triggered further analysis (G, H, I).
        }}
    \vspace{-3mm}
    \label{fig:case2-stock-step1}
\end{figure*}

\subsubsection{Quantitative Stock Trading}
In this case study, we collaborated with E$_3$, a junior quantitative stock trader specializing in short-term trading in the U.S. stock market.
\weikai{He has also participated in the interview in Sec.~\ref{sec:overview}}.
His goal was to identify stocks with rising prices using a stock price prediction model.
The training data consists of 119,416 samples collected from the U.S. stock market from April 2020 to April 2023, and the test data consists of 10,062 samples collected from May 2023 to August 2023. % from the subsequent three months (from May 2023 to August 2023).
Each sample represents the information of a stock at a specific time point, including two types of attributes~\cite{edwards2018technical}: 158 \emph{technical analysis attributes} and 99 \emph{fundamental attributes}.
The technical analysis attributes are derived from historical prices to evaluate and forecast financial market trends.
For example, \emph{STD60} measures the variance in stock prices over the preceding 60 days.
The fundamental attributes provide insights into a company's financial health and operational performance.
For example, \emph{revenueGrowth} reflects the company's revenue growth rate.
Based on the stock price fluctuation over the next seven days, the samples are categorized  into three classes: ``\textbf{increase},'' ``\textbf{decrease},'' and ``\textbf{stable}.'' 
% The class distribution is imbalanced, with ``increase,'' ``decrease,'' and ``stable'' comprising 14.9\%, 17.5\%, and 67.6\% of all samples, respectively.
Directly using all attributes to train the model can deteriorate its generalization ability due to attribute redundancy~\cite{htun2023survey}. %a stock price prediction 
Following the common practice, E$_3$ \jwrevision{selected attributes with an information coefficient larger than 0.05~\cite{goodwin1998information}, resulting in 140 attributes remaining.} 
%conducted feature selection by selecting the attributes with an information coefficient larger than 0.05~\cite{goodwin1998information}. As a result, there remained 140 attributes.
He then used these attributes to train a gradient boosted tree model with LightGBM~\cite{ke2017lightgbm} due to its superior performance and widespread adoption. %  in quantitative trading
\lizhen{The model was configured with 1000 trees and a maximum depth of 14.}
This model includes \textbf{81,000} rules but achieves an accuracy of only 56.26\%, with class-specific accuracy of 26.69\% for ``increase,'' 41.53\% for ``decrease,'' and 66.56\% for ``stable.''

\noindent\textbf{Overview}. 
Initially, E$_3$ wanted to verify whether the model utilized appropriate attributes for prediction. 
He checked the most frequently used attributes in the \textit{matrix view} and found the top-5 of them are technical analysis attributes (Fig.~\ref{fig:case2-stock-step1}(a)).
E$_3$ explained that these technical analysis attributes offered a more direct reflection of price fluctuations than fundamental attributes.
%Thus, 
\jwrevision{So,} the model relied more on these technical analysis attributes to make predictions.

Next, E$_3$ investigated whether the key attributes were correctly used.
He examined the most important attribute \emph{KLEN} in the first column (Fig.~\ref{fig:case2-stock-step1}A), \lizhen{which reflects the previous day's stock price range}.
He quickly found that the model tended to predict the stock price as ``stable'' when \emph{KLEN} was low.
This is reasonable because stocks with lower \emph{KLEN} are more likely to maintain stable prices in the next few days.
% He examined the first column corresponding to the most important attribute \emph{KLEN} (Fig.~\ref{fig:case2-stock-step1}A), \lizhen{which reflects the previous day's stock price range}.
% Upon examining the bottom of this column, he noticed that the height of the yellow bar was higher than others, which indicated that \emph{KLEN} was mostly used in the rules predicting ``stable'' (Fig.~\ref{fig:case2-stock-step1}B).
% Moreover, he found that the model tended to predict the stock price as ``stable'' when \emph{KLEN} was low.
% E$_3$ regarded it as reasonable because stocks with lower \emph{KLEN} are more likely to maintain stable prices in the next few days.

\noindent\textbf{Addressing biased predictions}.
When analyzing the attribute \emph{KLEN}, E$_3$ identified an exception: a rule made an ``increase'' prediction when \emph{KLEN} was low (Fig.~\ref{fig:case2-stock-step1}B).
In addition to \emph{KLEN}, this rule \jwrevision{used} %made predictions using 
three other attributes: \emph{RESI20}, \emph{industry}, and \emph{RESI60}.
%Upon examination of 
\jwrevision{Examining} the samples covered by this rule, he found that these samples had small \emph{KLEN}, medium \emph{RESI20}, and medium \emph{RESI60}, all of which indicated stable stock prices.
\jwrevision{However, the condition of \emph{industry=Bank} may be the reason for the prediction of ``increase.''} 
%Therefore, he suspected that the condition of \emph{industry=Bank} was crucial for the prediction of ``increase.''
E$_3$ commented that the economic cycles of different industries can vary a lot and lead to biased predictions.
Specifically, the banks associated with these samples experienced a growth period when \jwrevision{the} training data was collected, so the trained model tended to predict them as ``increase.''
However, such a pattern did not exist in the test samples and thus caused a performance drop.
To address this issue, he removed the attribute \jwrevision{\emph{industry}.} %\emph{industry} that caused biased predictions.
% For a similar reason, he also removed another industry-related attribute \emph{sector}.
\jwrevision{After retraining the model,} 
%After retraining the model with the remaining attributes, 
he observed an improvement in accuracy from 56.26\% to 56.52\%.
Specifically, on the samples with \emph{industry=Bank}, the accuracy increased from 48.90\% to 51.22\%.



\noindent\textbf{Improving model performance in ``increase.''}
As E$_3$'s primary goal was to find stocks with possibly rising prices to maximize profits, he focused on analyzing the attributes related to the ``increase'' class in the retrained model. 
\jwrevision{As shown in Fig.~\ref{fig:case2-stock-step1}C, he observed that \emph{STD60} was frequently used for the prediction of ``increase''.}
%As shown in Fig.~\ref{fig:case2-stock-step1}(b), he observed that \emph{STD60} was frequently used for the prediction of ``increase'', in the model, evidenced by the high green bar in the last row of the corresponding column (Fig.~\ref{fig:case2-stock-step1}D).
%This indicated that \emph{STD60} was critical to the prediction of ``increase.''
After investigating the rules using this attribute, he noticed that the rules with the conditions of larger \emph{STD60} consistently made predictions of ``increase'' (Fig.~\ref{fig:case2-stock-step1}D).
However, E$_3$ commented that a larger \emph{STD60} just meant a large fluctuation in stock prices over the past 60 days, which did not necessarily indicate an increasing stock price.
%Thus, a larger \emph{STD60} should not contribute to the prediction of ``increase.''
\jwrevision{Given the heavy reliance on this attribute to predict ``increase'' and the low prediction accuracy in this class (26.35\%),} 
%Given that the model heavily relied on this irrelevant attribute for predicting ``increase'' and the corresponding low accuracy in this class (26.35\%), 
E$_3$ concluded that \emph{STD60} was not a useful attribute for the prediction of this class and more attributes were needed.
%To complement useful attributes for predicting ``increase,'' %he generated 28 additional attributes using TA-lib
\lizhen{\jwrevision{He then} %he 
performed feature engineering by leveraging TA-lib~\cite{ta-lib}, an open-source tool, to generate \weikai{more} technical analysis attributes.}
After adding these attributes and retraining the model, the overall accuracy increased from 56.52\% to 58.35\%, and the class accuracy of ``increase'' increased from 26.35\% to 28.24\%.

%\begin{figure}[t]
%  \centering
%    \includegraphics[width=1\linewidth]{figures/stock2_revision.pdf}
%     \vspace{-2mm}
%        \caption{
        %Analyzing the retrained model with additional attributes: \lizhen{the importance of \textit{STD60} usage decreased (A), while \textit{NATR} became the most important one (B, C), which triggers further analysis of \textit{NATR} and related attributes (D, E). Another key attribute, \textit{VMA20}, associated with stability (F), was found redundant, with low \textit{NATR} identified as the crucial factor (G, H).}
 %       \jwrevision{Analyzing the retrained model with additional attributes. Note the decreased importance of the attribute \textit{STD60} (A), and the most important attribute \textit{NATR} (B), which triggers further analysis (D, E, H).}
  %      }
   % \vspace{-3mm}
    %\label{fig:case2-stock-step2}
%\end{figure}

To verify whether the newly added attributes were used correctly, E$_3$ examined the extracted rules again.
\weikai{The usage of \emph{STD60} decreased from 26 to 7 (Fig.~\ref{fig:case2-stock-step1}E), while a newly added attribute, \emph{NATR}, became the most frequently used (Fig.~\ref{fig:case2-stock-step1}F).
This attribute represents asset volatility.}
\jwrevision{A high \emph{NATR} indicates a large variation in stock prices. Sorting rules by \emph{NATR}, E$_3$ found that, indeed, high \emph{NATR} values are associated with ``increase'' or ``decrease'' predictions, while low \emph{NATR} values are associated with ``stable'' predictions. (Fig.~\ref{fig:case2-stock-step1}G)} 
% First, \emph{STD60} was used less frequently (Fig.~\ref{fig:case2-stock-step2}A), with only 7 of 80 rules using this attribute, compared with the previous 26 of 80.
% \lizhen{Second, the newly added attribute, \emph{NATR}, which represents asset volatility, became the most frequently used (Fig.~\ref{fig:case2-stock-step2}B).
%Many rules containing \emph{NATR} predicted ``increase'' or ``decrease''.
%After sorting rules by \emph{NATR}, E$_3$ found that all the rules with high \emph{NATR} made the prediction of ``increase'' or ``decrease'' (Fig.~\ref{fig:case2-stock-step1}H).
%\lizhen{Given that} a larger \emph{NATR} indicates a larger degree of variation in stock prices,
\lizhen{E$_3$} wondered how other attributes collaborated with %the condition of 
high \emph{NATR} to predict the \jwrevision{``increase'' or ``decrease.''} %change of the stock price.
Therefore, he explored %those 
\jwrevision{rules} with the condition of high \emph{NATR}. % \lizhen{using dynamic hierarchy}.
\jwrevision{The neighborhood was dynamically constructed, where} 
%\lizhen{In the dynamically constructed neighborhood}, 
he found that \emph{revenueGrowth}, \jwrevision{the growth of the profit rate,} %which represents the growth of the profit rate, 
was frequently used in these rules (Fig.~\ref{fig:case2-stock-step1}H).
% \lizhen{This information provided a more detailed understanding of the relationship between high \textit{NATR} and stock price changes.}
% He also found \lizhen{a clear pattern} that high \emph{revenueGrowth} mostly led to an ``increase'' prediction, while low \emph{revenueGrowth} mostly led to a ``decrease'' prediction.
\weikai{The ordering result reveals a clear pattern that} high \emph{revenueGrowth} mostly led to an ``increase'' prediction, while low \emph{revenueGrowth} mostly led to a ``decrease'' prediction.
This observation was consistent with his experience.


\noindent\textbf{Removing redundant attributes}. 
During further exploration, E$_3$ identified some redundant attributes for prediction.
For example, \emph{VMA20}, \lizhen{which indicates the average trading volume in the preceding 20 days}, was recognized as an important attribute and ranked \jwrevision{the} ninth among \jwrevision{the} over 100 attributes (Fig.~\ref{fig:case2-stock-step1}I).
However, in the rules using this attribute, both \jwrevision{low and high} %small and large 
\emph{VMA20} resulted in the predictions of ``stable'' (Fig.~\ref{fig:case2-stock-step1}J), \jwrevision{which seemed to suggest the value of VMA20 does not affect the prediction}. 
%Thus, E$_3$ hypothesized that \emph{VMA20} did not actually affect the predictions of these rules.
To further analyze these rules, %he 
\jwrevision{E$_3$} pinned \jwrevision{VMA20} %this attribute 
to the first column and sorted \jwrevision{rules based on it.} %the rules based on \emph{VMA20}.
He %then 
found that \jwrevision{all the rules using VMA20 also used NATR and had low NATR values. As low NATR indicates a small variation in stock prices, E$_3$ believed it was the actual reason behind the predictions of these rules, and \emph{VMA20} was redundant. He proposed to remove \emph{VMA20}.} 
%all of them had small \emph{NATR} (Fig.~\ref{fig:case2-stock-step1}L), which was the actual reason behind their predictions. Therefore, he believed that \emph{VMA20} was redundant and proposed to remove it.
Similarly, he removed another eight redundant attributes.
After retraining the model, its accuracy was improved to 59.20\%.

Finally, E$_3$ employed the final model for simulated trading.
The trading strategy involved selecting 20 stocks predicted to be the most likely to increase in each 7-day trading cycle over a period of 3 months.
Backtesting proved that this trading strategy produced an excess return of 48.7\% with a maximum draw down of 5.0\%.
E$_3$ was pleased with this performance and said the comprehensive understanding of this model made him more confident in employing \jwrevision{the model} %it 
for real-world trading.




\subsection{Expert Feedback and Discussion}
After the case studies, we conducted semi-structured interviews with each of the six experts \lizhen{(E$_1$-E$_6$) introduced in Sec.~\ref{sec:overview}-A.}
%E$_1$–E$_3$ collaborated in the case studies, while E$_4$–E$_6$ were newly engaged in the interview process.
%, including E$_1$--E$_3$ who collaborated in the case studies, and E$_4$--E$_6$ who were newly invited. 
%E$_4$ is a fund manager, E$_5$ is a vice president of a bank branch, and E$_6$ is a doctoral student majoring in visualization and machine learning with 5 years of experience. 
% We conducted a semi-structured interview with each expert.
% For E$_4$-E$_6$, we first introduced {\system} and presented the case studies.
%\weikai{%Since 
%\jwrevision{As} E$_4$-E$_6$ were not involved in the case studies, we first introduced {\system} and presented the case studies \jwrevision{to them}.} 
\lizhenrev{E$_4$-E$_6$ were not involved in the case studies. These newly involved experts included a fund manager with two years of experience (E$_4$), a vice president at a commercial bank branch (E$_5$), and a machine learning researcher with five years of experience (E$_6$). For E4-E6, we spent the initial 20 minutes introducing {\system} and presenting the case studies. Each expert then used {\system} for model understanding and verification tasks. It took 5-15 minutes for them to become familiar with the interactions and conduct analysis.} We concluded with a discussion on {\system}’s advantages and limitations. Each interview lasted 35-60 minutes.



\subsubsection{Usability}
Overall, the experts are quite satisfied with {\system}.

\noindent\textbf{Learning curve}.
The experts consider {\system} \jwrevision{is} %to be 
easy to use.
They like that the matrix view takes a format similar to a data table and naturally supports table operations, such as sorting and swapping.
This familiar design has enhanced their analysis efficiency.
They also indicate that using {\system} enables them to quickly understand the model, which has increased their trust in the model and their confidence in decision-making. \weikai{
Specifically, they expressed satisfaction with
the dynamic hierarchy, which enables them to analyze different subsets of rules on demand.
The experts also value the ease of finding anomalous rules using {\system}.
As E$_2$ commented, ``Different from RuleMatrix~\cite{ming2018rulematrix} and ExplainableMatrix~\cite{neto2020explainable}, this tool automatically recommends some unusual rules, which help me quickly identify potential issues in the model and make interventions accordingly.''}


\noindent\weikai{\noindent\textbf{Scalability}.
Matrix visualizations often face the scalability issue due to the limited number of rows and columns \jwrevision{that can be displayed}%they can display
~\cite{ming2017understanding,yang2022diagnosing}.
To tackle this issue, {\system} 1) organizes a large rule set into a hierarchy and dynamically selects representative rules to display, and 2) sorts attributes by importance and divides them into pages.
These two strategies are effective because \lizhenrev{tree ensemble models typically select a smaller set of key attributes for decision making~\cite{breiman2001random}, and} users usually focus on a small subset of \lizhenrev{representative rules and key attributes for initial analysis.}
In addition, our tool can \jwrevision{easily be} %also be easily 
extended to handle other scalability issues. \jwrevision{For example,} 
for %categorical 
attributes with thousands of categories, we can employ alternative feature transformation methods, such as Target Encoding~\cite{geron2022hands}, which replaces each category with a single numerical value representing its statistical correlation to the target variable.
For classification tasks involving more than 10 classes, we can hierarchically organize classes and dynamically assign colors during user exploration ~\cite{chen2024dynamic}.}

\noindent\weikai{\noindent\textbf{Extensibility}.
While {\system} is primarily designed for tree ensemble classifiers, it can be easily extended for regression models.
To achieve this, users simply need to substitute the classification-specific loss with a regression-specific loss during model reduction and employ sequential color schemes to encode the regression values of each rule.
In addition, E$_6$ also pointed out that {\system} can be used to explain other models beyond tree ensemble models: ``Similar to RuleMatrix~\cite{ming2018rulematrix}, this tool supports the analysis of other machine learning models using model surrogate techniques.
This greatly extends the applicability of the tool.''}


\subsubsection{Limitations}

In addition to the positive feedback, the experts also point out several limitations that offer directions for future research.

\noindent\textbf{Online model update}. 
In the current analysis, after the experts identify problems and make corrections, they need to retrain the model and load it back into the system. The experts highlighted that the ability to incrementally update parts of the model online to examine the result would help improve the analysis efficiency. Exploring methods for incrementally updating the model and effectively visualizing the changes presents an interesting research direction.

\noindent\textbf{What-if analysis}.
Another interesting direction is the what-if analysis of rules. E$_6$ suggested allowing examination of how different rule conditions impact the output. However, further exploration is needed on how to use what-if analysis to more accurately guide experts in improving the model.
This research will focus on understanding model rules and making corresponding modifications. We plan to gather more specific requirements from experts to guide future research.

\noindent\textbf{Algorithm efficiency}.
%The current efficiency of the model reduction algorithm is not high enough. The runtime varies from tens of seconds to a few hours depending on the model complexity and data size. Considering the model reduction is operated offline, the experts think such a time consumption is acceptable.
% \lizhen{The current efficiency of the model reduction algorithm,  which constitutes a major component of the offline preprocessing in our tool, is not high enough. The runtime of model reduction varies from tens of seconds to a few hours, depending on the model complexity and data size. For our largest scenario, it can take 3-4 hours, while for the model in Sec.~\ref{sec:evaluation}-A, it takes up to 30 minutes. However, since model reduction is performed offline after training, experts find this time acceptable, as they are willing to invest it for the benefits in the big data era. In contrast, the online analysis in our tool can be completed within seconds, supporting users' real-time analysis.}
The current efficiency of the model reduction algorithm \weikai{is not as high as desired.
The running time ranges from tens of seconds to a few hours, depending on the model complexity and data size.
For example, it takes around 1 minute for the model in the first case study and takes 3-4 hours in the second case study.}
\lizhen{However, since model reduction is performed offline,  %after training, 
experts find this time acceptable, as they are willing to \jwrevision{trade off time for scalability}  %invest in it for the benefits 
in the big data era.
}
% In contrast, the online analysis in our tool can be completed within seconds,  supporting users’ real-time analysis.
%
\weikai{Nevertheless, accelerating this process allows experts to start their analysis at the earliest opportunity.}
The bottlenecks here lie in the grid search for the algorithm parameters and linear programming in Sec.~\ref{sec:reduction}.
In the future, we will design a method for quickly determining algorithm parameters, and simplify the linear programming by retaining more important constraints and variables to accelerate problem solving.



==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS, incl. InfoVis, SciVis, VAST)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)

